A Mechanism for Participatory Budgeting With Funding Constraints and Project Interactions

Participatory budgeting (PB) has been widely adopted and has attracted significant research efforts; however, there is a lack of mechanisms for PB which elicit project interactions, such as substitution and complementarity, from voters. Also, the outcomes of PB in practice are subject to various minimum/maximum funding constraints on 'types' of projects. We propose a novel preference elicitation scheme for PB which allows voters to express how their utilities from projects within 'groups' interact. We consider preference aggregation done under minimum and maximum funding constraints on 'types' of projects, where a project can have multiple type labels as long as this classification can be defined by a 1-laminar structure (henceforth called 1-laminar funding constraints). Overall, we extend the Knapsack voting model of Goel et al. [26] in two ways - enriching the preference elicitation scheme to include project interactions and generalizing the preference aggregation scheme to include 1-laminar funding constraints. We show that the strategyproofness results of Goel et al. [26] for Knapsack voting continue to hold under 1-laminar funding constraints. Moreover, when the funding constraints cannot be described by a 1-laminar structure, strategyproofness does not hold. Although project interactions often break the strategyproofness, we study a special case of vote profiles where truthful voting is a Nash equilibrium under substitution project interactions. We then study the computational complexity of preference aggregation. Social welfare maximization under project interactions is NP-hard. As a workaround for practical instances, we give a fixed parameter tractable (FPT) algorithm for social welfare maximization with respect to the maximum number of projects in a group when the overall budget is specified in a fixed number of bits.

==> greedy1.tex <==
\begin{algorithm}[t]
\SetAlgoLined
 \SetAlgorithmName{Greedy Algorithm}{} 

Initialize $Q \leftarrow \emptyset$\\
\For{$i = 1,2, \ldots, B$}{

%$p^* = \argmax_{\rho \in [m]\setminus Q} U(Q\cup \{\rho\}) $ \\
$Q \leftarrow Q \cup \Big\{   \argmax\limits_{\rho \in [m]\setminus Q} ~~ U(Q\cup \{\rho\})   \Big\}$ 


%$p^* = \argmax_{\rho \in [m]\setminus Q} U(Q\cup \{\rho\}) $ \\
%$Q \leftarrow Q \cup \{p^*\}$
}
    \caption{Input: $(Z,B,V)$, Output: $Q$}
\label{alg:greedy}
\end{algorithm}


==> proof_NE.tex <==
%This proof is in two parts. 
%First, we give Lemma~\ref{lem:greedy}, which says that the Greedy Algorithm~\ref{alg:greedy} solves SWM-PB under Assumptions~\ref{ass:integer},~\ref{ass:no_comp},~\ref{ass:unitcost}, and~\ref{relaxed_assumption:votes} when at most one voter is not voting truthfully (and their vote may not satisfy Assumption~\ref{relaxed_assumption:votes}). The proof of Lemma~\ref{lem:greedy} is in the Appendix \S~\ref{proof:lem_greedy}.

\begin{proof}
Let $V_{-i}$ denote the vote profile of voters other than voter $i.$ Let voter $i's$ truthful vote be $(f^i,s^i)$ and their reported vote be $(\hat{f}^i, \hat{s}^i).$ We drop the budget constraint of $\sum_{g \in [r]} \hat f_g^i \leq B$ for $\hat f^i_g$ and show that even without the constraint, truthful voting is a weakly dominant strategy for voter $i$ if $V_{-i}$ satisfies Definition~\ref{def:vote_profiles}. Note that $i$'s truthful vote satisfies the budget constraint by the model's design.
%
%Let $b_{\rho}$ denote the amount of funds allotted to group $\rho$ in SWM-PB.  %Let $h^*_B$ denote the cutoff marginal social utility for a unit of funding to be assigned to any group. %Denote the set of funded projects under SWM-PB by $Q$.
When $b$ units of funds are allotted to group $g,$ recall that $\mathcal{U}_{\{g\}}(b)$ denotes the reported (not necessarily ``true'') social welfare 
%\footnote{This may be different from the \emph{true} social utility since voter $i$ might not report their true vote.}  
of an optimal bundle from group $g.$

For any group $g \in [r]$, consider the scenario where voter $i$ has set $\{(\hat{f}^i_{\rho}, \hat{s}^i_{\rho}) \}_{ \rho \neq g, \rho \in [r]}$ for the other groups and is deciding their vote for group $g$, with default initialization of $(\hat f^i_g = 0, \hat s_g^i = \emptyset)$. We show that for any $\{(\hat{f}^i_{\rho}, \hat{s}^i_{\rho}) \}_{ \rho \neq g, \rho \in [r]}$, voter $i$'s truthful vote $(f_g^i,s_g^i)$ on group $g$ is weakly dominant. % over all possible reports $(\hat f_g^i, \hat s_g^i).$  
%
%Voter $i$'s vote on group $g$ can only increase its social utility $\mathcal{U}_g(b)$ for all $b$.
Consider the following exhaustive set of cases over the type of the group and voter $i$'s utility from it.

\begin{itemize} [ leftmargin = 0.15cm, align=left]
    \item [1.] \textbf{Voter $i$ derives no utility from group $g$, i.e., $f_g^i = 0$.}  Setting $\hat f_g^i > 0$ and $\hat s_g^i \neq \emptyset$ can only increase $\mathcal{U}_{\{g\}}(b)$ for any $b$. This can only reduce the funding from the other groups. Per Lemma~\ref{lem:greedy}, this cannot cause the addition of any new project in the outcome $Q$ from outside of group $g$ and hence cannot increase voter $i$'s utility. Therefore, setting $\hat f_g^i = 0$ and $\hat s_g^i = \emptyset$ is a weakly dominant strategy for voter $i.$

    
    \item [2a.] \textbf{Group $g$ is a group of contradictory projects.} Let $p$ be the project in $s_g^i.$ By design, the reported social utilities of projects in contradictory groups are additively separable. Therefore,  to solve SWM-PB, each project from group $g$ can be considered a separate singleton group.
   
    If voter $i$ votes truthfully, they maximize the reported social welfare of project $p$. This may get project $p$ included in $Q$ if it is not already present. Per Lemma~\ref{lem:greedy}, one project is eliminated from $Q$ if project $p$ gets included. Voter $i$'s utility can, therefore, not decrease.

    There are two ways for voter $i$ to lie: by giving $\hat f_g^i = 0$ or by giving $(\hat f_g^i = 1, \hat s_g^i = \{p^\prime\})$ where $p^\prime \neq p.$  In the former, their utility doesn't change. In the latter, they can only lose 1 unit of utility if $p^\prime$ gets included in $Q$ by replacing a project from which $i$ gets utility. Overall, it is impossible to increase utility by lying.
    %
    This shows that the truthful vote $\hat f^i_g = 1, \hat s_g^i = \{p\}$ is  a weakly dominant strategy for voter $i$.
    \item [2b.] \textbf{Group $g$ is a group of independent projects.}
    
    \textit{Case I:} $\hat f_g^i = |\hat s_g^i|.$ ($\hat f_g^i > |\hat s_g^i|$ is identical to $\hat f_g^i = |\hat s_g^i|$ for the utility function). In this case, the reported social utilities of the different projects from group $g$ are additively separable.  %To solve SWM-PB, each project from group $g$ can be considered a separate singleton group. 
    Adding a project $p$ to $\hat s_g^i$  can cause its inclusion to $Q$ while removing exactly one project from $Q$ as per Lemma~\ref{lem:greedy}. If project $p$ is in $ s_g^i$ then this can only increase $i$'s utility, and if project $p \notin s_g^i$, then this can only decrease $i$'s utility.



    \textit{Case II:} $\hat f_g^i < |\hat s_g^i|.$ For the purpose of SWM-PB, this vote is equivalent to truncating $\hat s_g^i$ to the top $\hat f_g^i$ projects in it as per their social utilities in $V_{-i}$ and the tie-breaking order. %With this truncation, 
    We now have the same problem as in \textit{Case I}. Adding all of $s_g^i$ (and no projects from outside of it) in the ``truncated'' $\hat s_g^i$  is, therefore, a weakly dominant strategy. This corresponds precisely to truthful voting.
        
    \item [2c.] \textbf{Group $g$ is a group of substitute projects.}
   % Recall that the votes is $V_{-i}$ satisfy Assumption~\ref{relaxed_assumption:votes} and 
   There is a partition $\Lambda_g = \{\lambda_{g,k}\}_{k \in [q_g]}$ of $z_g$ such that every vote in $V_{-i}$ approves projects from at most one of $\lambda_{g,k}.$ Let $\lambda_{g,*}$ be the subgroup from which voter $i$ derives utility and $\lambda_{g,*} = \{\rho_1, \rho_2, \ldots, \rho_{|\lambda_{g,*}|}\}$ with subscript denoting the rank of the projects as per the partial  order in Definition~\ref{def:vote_profiles}.

    For any $\hat f_g^i > 0$ and $\hat s_g^i \subseteq \lambda_{g,*}$, expanding $\hat s_g^i$ by approving projects from $z_g\setminus\lambda_{g,*}$ can only include additional projects from $z_g\setminus\lambda_{g,*}$ to the outcome $Q$.
    This follows from Lemma~\ref{lem:greedy}. 
    This will remove projects already in $Q$, and $i$'s utility cannot increase. Therefore, not approving any project from $z_g\setminus\lambda_{g,*}$ is a weakly dominant strategy.

    It now remains to decide $\hat f_g^i$ and $\hat s_g^i \subseteq \lambda_{g,*}.$

Let $s_g^i$ have projects from rank $1$ to $\psi.$ Naturally $f_g^i \leq \psi.$  Let $b^*$ be the amount of funding allotted to subgroup $\lambda_{g,*},$ if voter $i$ votes truthfully in $g$. The top $b^*$ rank projects from $\lambda_{g,*}$ (up to tie-breaking) get funded. This is because, in any set of projects, if we replace a lower-ranked project $p_l$ with a higher-ranked project $p_h$, then the reported social welfare cannot decrease since all voters who get utility from project $p_l$ also get the same utility from project $p_h$.
In this outcome, voter $i$'s utility from group $g$ is $\min(f^i_g, b^*).$

For deviation $(\hat f^i_g, \hat s^i_g),$ let $b$ units of funds be allocated to $\lambda_{g,*}.$ We consider two cases of $b^*$ ($\geq$ or $< f^i_g$) and show that in both cases, there doesn't exist a profitable deviation.


\textit{Case I: $b^* \geq f^i_g$.} The utility of voter $i$ from the group is capped at $f^i_g.$ 
 If $b \geq b^*,$ then the utility from other groups can only decrease as per Lemma~\ref{lem:greedy}, but that from group $g$ cannot increase.
Whereas, if $b < b^*,$  the utility of voter $i$ from group $g$ must decrease by at least $b^*-b.$ This is because only those projects can be removed from the outcome $Q$ whose approval is removed by voter $i$ in the deviation. 
The projects which were in $Q$ without $i$'s contribution to their marginal social welfare, remain in $Q$ despite any deviation in voter $i$'s vote. $i$'s utility from outside the group can increase by at most $b^*-b$. Overall, therefore, $i$'s utility cannot increase.

\textit{Case II: $b^* < f^i_g$.} If $b \leq b^*,$  the utility of voter $i$ from group $g$ decreases by at least $b^*-b.$ This is because $b$ projects can give at most $b$ utility. The utility from outside the group can increase by at most $b^*-b$ per Lemma~\ref{lem:greedy}.
Also, even for $b>b^*,$ voter $i$ cannot increase its utility from the group because their utility-increasing projects from the groups have the maximum possible reported marginal social welfare in the truthful vote itself, and per Lemma~\ref{lem:greedy}, they cannot be included to $Q$ at a lower marginal social welfare. 
\end{itemize}
\end{proof}

==> proof_gf.tex <==
\subsection{Proofs of Lemma~\ref{lem:greedy-gf} and Theorem~\ref{thm:nash-equilibrium-gf}}\label{sec:proof_greedy_gf}

\subsubsection{Proof of Lemma~\ref{lem:greedy-gf} }
\begin{proof}
The proof is very similar to that of Lemma~\ref{lem:greedy}. Same as in the proof of Lemma~\ref{lem:greedy}, for contradictory groups, even under a deviation
from truthful voting (that is, one vote does not follow Definition~\ref{def:vote_profiles}), the reported social welfares of all projects are additively
separable per the design of the mechanism and therefore greedy allocation is optimal. This holds even under funding constraints.

For non-contradictory groups, we consider a set of five exhaustive cases in the proof of  Lemma~\ref{lem:greedy} -- here too we consider the same set of cases. In each case, the arguments in the proof are for the decisions of the aggregation algorithm in each group separately. Further, in each case, the proof holds for all levels of funding allocated to each group. Therefore it also holds under the funding constraints.
\end{proof}

\subsubsection{Proof of Theorem~\ref{thm:nash-equilibrium-gf}}

\begin{proof}
    The proof follows along similar lines as that of Theorem~\ref{thm:nash-equilibrium-gf}. The key new detail is that when a group's funding is restricted by funding constraints, even then a strategic deviation cannot improve a voter's true utility.

    We first recall the notation defined in the proof of Theorem~\ref{thm:nash-equilibrium-gf}.

     $V_{-i}$ denotes the vote profile of all voters other than voter $i.$  Voter $i's$ truthful (unobservable) vote is denoted by $(\hat{f}^i, \hat{s}^i)$.  Their reported vote is $(f^i,s^i)$.
When $b$ units of funds are allotted to group $g,$ recall that $\mathcal{U}_{\{g\}}(b)$ denotes the reported social welfare   
of an optimal bundle of size $b$ from group $g.$


For any group of projects $g \in [r]$, we consider the scenario where voter $i$ sets $\{(f^i_{\rho}, s^i_{\rho}) \}_{ \rho \neq g, \rho \in [r]}$ for the remaining groups and is deciding their vote for group $g$, with default initialization of $(\hat f^i_g = 0, \hat s_g^i = \emptyset)$. 
In the proof, we study how voter $i$'s true utility changes relative to the outcome in this state on setting their vote in group $g$.

We show that for any report $\{(f^i_{\rho}, s^i_{\rho}) \}_{ \rho \neq g, \rho \in [r]}$, voter $i$'s truthful vote $(\hat f_g^i,\hat s_g^i)$ on group $g$ is a weakly dominant strategy. This is sufficient to prove the theorem.

Consider the following exhaustive cases on the group and voter $i$'s utility.


    %\item [1.] 
    \textbf{1. Voter $i$ derives no utility from group $g$:}  Setting $ f_g^i > 0$ and $ s_g^i \neq \emptyset$ cannot decrease $\mathcal{U}_{\{g\}}(b)$ for any $b$ regardless of whether the funding constraints are tight or not. This can only reduce the funding from the other groups per Lemma~\ref{lem:greedy-gf}. Per Lemma~\ref{lem:greedy-gf}, this cannot cause the addition of any new project in the outcome $Q$ from outside of group $g$ and hence cannot increase voter $i$'s true utility. Therefore, truthful voting is a weakly dominant strategy.

    
    %\item [2a.]
    \textbf{2a. Group $g$ is of contradictory projects.} Let $p$ be the project in the true vote's approval set $\hat s_g^i.$ Since the utilities of projects in contradictory groups are additively separable, each project from group $g$ can be considered a separate singleton group.
   
    If voter $i$ votes truthfully, they maximize the reported SW of project $p$. This may only get project $p$ included in $Q$ if not already present. If $p$ is already present in $Q,$ this makes no change to the outcome, regardless of the funding constraints being active or not in the group. Per Lemma~\ref{lem:greedy-gf}, one project is eliminated from $Q$ if $p$ gets included. Voter $i$'s true utility, therefore, cannot decrease.

    There are two ways for voter $i$ to lie: by giving $ f_g^i = 0$ or $( f_g^i = 1, s_g^i = \{p^\prime\})$ where $p^\prime \neq p.$  In the former, their true utility doesn't change. In the latter, they can only lose 1 unit of true utility if $p^\prime$ gets into $Q$ by replacing a project from which $i$ gets true utility. Overall, it is impossible to increase true utility by lying in this case.
    %
   % This shows that the truthful vote $\hat f^i_g = 1, \hat s_g^i = \{p\}$ is  a weakly dominant strategy for voter $i$.
   
    %\item [2b.]
    \textbf{2b. Group $g$ is a group of independent projects per Definition~\ref{def:vote_profiles}.}
    
    \underline{\textit{Case I:}} $ f_g^i = | s_g^i|.$ (see that $ f_g^i > |s_g^i|$ is identical to $ f_g^i = | s_g^i|$ for the utility function, and therefore we need not consider it separately). In this case, the reported social welfare of the projects in group $g$ are additively separable.  %To solve SWM-PB, each project from group $g$ can be considered a separate singleton group. 
    Adding a project $p$ to $s_g^i$  can only cause its inclusion to $Q$ while removing exactly one project from $Q$ as per Lemma~\ref{lem:greedy-gf}. This holds regardless of the funding constraints. If project $p$ is in $\hat s_g^i$ then this can only increase $i$'s true utility, and if project $p \notin \hat s_g^i$, then this can only decrease $i$'s true utility. Therefore only including the projects from $\hat s_g^i$ in $s_g^i$ is a weekly dominant strategy.

    \underline{\textit{Case II:}} $f_g^i < |s_g^i|.$ For the purpose of the Greedy Algorithm~\ref{alg:greedy-gf}, this vote is equivalent to truncating $s_g^i$ to the top $f_g^i$ projects per their social utilities in $V_{-i}$ and the tie-breaking order. %With this truncation, 
    We now have the same problem as in \textit{Case I}. Adding all of $\hat s_g^i$ and no projects from outside of it in the ``truncated'' $s_g^i$  is, therefore, a weakly dominant strategy. This corresponds precisely to truthful voting in the group.
        
   % \item [2c.]
   \textbf{2c. Group $g$ is a group of substitute projects per Definition~\ref{def:vote_profiles}.}
   % Recall that the votes is $V_{-i}$ satisfy Assumption~\ref{relaxed_assumption:votes} and 
   Recall that we defined the following notation for the order in $z_g.$ There is a partition $\Lambda_g = \{\lambda_{g,k}\}_{k \in [q_g]}$ of $z_g$ such that there is a strict total order within each $\lambda_{g,k}.$ Every voter in $V_{-i}$ approves projects from at most one of $\lambda_{g,k}$ per Definition~\ref{def:vote_profiles}.  Let $\lambda_{g,*}$ be the subgroup from which voter $i$ derives true utility.% 
   
    For any $f_g^i > 0$ and $s_g^i \subseteq \lambda_{g,*}$, untruthfully expanding $s_g^i$ by approving projects from $z_g\setminus\lambda_{g,*}$ can only include additional projects from $z_g\setminus\lambda_{g,*}$ to the outcome $Q$.
    This follows from Lemma~\ref{lem:greedy-gf}. This is regardless of the funding constraints.
    This will remove an equal number of projects already in $Q$, and $i$'s true utility cannot increase. Therefore, not approving any project from $z_g\setminus\lambda_{g,*}$ is a weakly dominant strategy.

    It now remains to decide $ f_g^i$ and $s_g^i$ such that $s_g^i \subseteq \lambda_{g,*}.$

Let in the true vote, $\hat s_g^i$ have projects from rank $1$ to $\psi$ in $\lambda_{g,*}.$ Setting $\hat f_g^i \geq \psi$ is equivalent to $\hat f_g^i = \psi$ for the utility function, so we  consider only the case of $\hat f_g^i \leq \psi.$ 

Consider the case where voter $i$ votes truthfully in group $g.$ Let $b^*$ funding be allotted to $\lambda_{g,*}$. Note that under funding constraints, $b^*$ can be at most $B^{\max}_q$ where $q$ is the 'type' of group $g$. The minimum funding constraint does not apply directly to the subgroup  $\lambda_{g,*}$ since it may be across multiple groups and subgroups.
 
 In this case, the top $b^*$ rank projects from $\lambda_{g,*}$ (up to tie-breaking) get funded.
This is because, in any outcome, if we replace a lower-ranked project $p_l$ with a higher-ranked project $p_h$, the social welfare cannot decrease since, per Definition~\ref{def:vote_profiles}, all voters who get utility from $p_l$ also get the same utility from $p_h$.
In this outcome, voter $i$'s utility from group $g$ is $\min(f^i_g, b^*).$

For a deviation $(f^i_g, s^i_g),$ let $b$ funds be allocated to $\lambda_{g,*}.$ We consider two cases of $b^*$  relative to the funding voter $i$ would put in group $g$ in their true vote, i.e., ($b^* \geq$ or $< \hat f^i_g$). We show that there is no profitable deviation in either case, even in the presence of funding constraints.


 \underline{\textit{Case I: $b^* \geq \hat f^i_g$.}} The true utility of voter $i$ from the group is capped at $\hat f^i_g.$ 
 If $b \geq b^*,$ then the true utility from other groups can only decrease on making a deviation (per Lemma~\ref{lem:greedy}), but that from group $g$ cannot increase.
Whereas, if $b < b^*,$  the true utility of voter $i$ from group $g$ must decrease by at least $b^*-b.$ This is because only those projects can be removed from the outcome $Q$ whose approval is removed by voter $i$ in the deviation. 
The projects which were in $Q$ without $i$'s contribution to their marginal social utility, remain in $Q$ despite any deviation in voter $i$'s vote. Voter $i$'s true utility from outside the group can increase by at most $b^*-b$. Overall, therefore, $i$'s true utility cannot increase.



\underline{\textit{Case II: $b^* < \hat f^i_g$.}} If $b \leq b^*,$  the true utility of voter $i$ from group $g$ decreases in this deviation by at least $b^*-b.$ This is because $b$ projects have at most $b$ utility. The utility from outside the group can increase by at most $b^*-b$ per Lemma~\ref{lem:greedy}.
Also, even for $b>b^*,$ voter $i$ cannot increase their true utility from the group because their utility-producing projects from the groups have the maximum possible reported marginal social utility in the true vote itself, and per Lemma~\ref{lem:greedy}, they cannot be included to $Q$ at a lower marginal social utility. 

Note that in this argument we did not assume anything regarding the values of $b$ and $b^*$ relative to the funding constraints. The arguments follow for all possible $b$ and $b^*$  and that is true even under funding constraints. This completes the proof.
\end{proof}

